ISB-NMPC: Interception-Oriented Spherical-Bearing Nonlinear Model Predictive Control for Quadrotors

Quadrotor interceptors equipped with strapdown cameras offer a low-cost solution for physically countering unauthorized UAVs. However, this configuration inherently couples vehicle maneuvering and camera pointing, creating a conflict between rapid closing and maintaining target visibility. We present interception-oriented spherical-bearing nonlinear model predictive control (ISB-NMPC), which couples spherical-bearing prediction with nonlinear quadrotor dynamics to jointly optimize target-directed closing motion and visibility. An attitude-compensated extended Kalman filter on S^2 estimates target bearing motion, compensates for perception delay, and predicts target bearings to guide scale-adaptive detection. Across 30 paired simulation trials, ISB-NMPC achieves an interception success rate of 86.7%, the highest among the evaluated controllers, with a mean per-trial target-visible time of 99.11%. Outdoor flights demonstrate acquisition of a 30 cm target at approximately 150 m, with interceptor speed reaching 17 m/s in the long-range flight and approximately 14 m/s while pursuing a quadrotor-towed maneuvering target. The software and hardware are open source at https://github.com/HOLYNOTBAD/ISB-NMPC and https://github.com/HOLYNOTBAD/holydrone, respectively.

==> image/bio/biographies.tex <==
% Author biographies in manuscript order; source text and portraits are in image/bio.
% Crop each portrait to the same 4:5 display box without stretching the source image.
\newcommand{\biophoto}[3]{%
  \includegraphics[width=1in,height=1.25in,trim=0 #2 0 #3,clip]{#1}}


\begin{IEEEbiography}[{\biophoto{image/bio/hongli.png}{11.5bp}{11.5bp}}]{Li Hong}
received the B.S. degree in control science and engineering from Shen Yuan Honors College, Beihang University, Beijing, China, in 2026, where he is currently pursuing the Ph.D. degree in control science and engineering. His main research interests include UAV navigation, planning, and control.
\end{IEEEbiography}

\begin{IEEEbiography}[{\biophoto{image/bio/liulinkai.jpg}{26.25bp}{26.25bp}}]{Linkai Liu}
is currently pursuing the Ph.D. degree in Navigation, Guidance and Control at the School of Automation Science and Electrical Engineering, Beihang University (formerly Beijing University of Aeronautics and Astronautics), Beijing, China. He received the B.S. degree in Intelligent Flight Vehicle Technology from Beihang University in 2025. His main research interests include vision-based guidance and control, and autonomous aerial robotics.
\end{IEEEbiography}

\begin{IEEEbiography}[{\biophoto{image/bio/renxiangyu.jpg}{9.57bp}{9.57bp}}]{Xiangyu Ren}
is currently pursuing the master's degree in control engineering with the School of Automation Science and Electrical Engineering, Beihang University, Beijing, China. His research interests include aerial robotics.
\end{IEEEbiography}

\begin{IEEEbiography}[{\biophoto{image/bio/lvshuli.png}{1.75bp}{1.75bp}}]{Shuli Lv}
received the B.S. degree in control science and engineering from Shen Yuan Honors College, Beihang University, Beijing, China, in 2022. He is currently pursuing the Ph.D. degree in control science and engineering with the School of Automation Science and Electrical Engineering, Beihang University. His main research interests include UAV navigation, planning, and control.
\end{IEEEbiography}

\begin{IEEEbiography}[{\biophoto{image/bio/minchen.jpg}{99bp}{99bp}}]{Chen Min}
received the B.S. degree in control science and engineering from Shen Yuan Honors College, Beihang University, Beijing, China, in 2025. He is currently working toward the Ph.D. degree in control science and engineering with Shen Yuan Honors College, Beihang University, Beijing, China. His main research interests include UAV navigation, planning, and control.
\end{IEEEbiography}

\begin{IEEEbiography}[{\biophoto{image/bio/wuchunjiang.jpg}{96.125bp}{96.125bp}}]{Chunjiang Wu}
received the B.S. degree in automation from North China Electric Power University, China, in 2023, and the M.S. degree in control science and engineering from the School of Automation Science and Electrical Engineering, Beihang University, Beijing, China, in 2026. He is currently pursuing the Ph.D. degree in low-altitude intelligent navigation technology at the Hangzhou International Innovation Institute of Beihang University, Hangzhou, China. His research interests include visual recognition and embodied intelligence.
\end{IEEEbiography}


\begin{IEEEbiography}[{\biophoto{image/bio/zhangyujun.jpg}{53.625bp}{53.625bp}}]{Yujun Zhang}
is currently pursuing the Ph.D. degree in Control Science and Engineering at Shen Yuan Honors College, Beihang University, Beijing, China. She received the B.S. degree in Automation from Beihang University in 2026. Her research interests include pursuit-evasion games, multi-UAV cooperative planning, and autonomous aerial robotics.
\end{IEEEbiography}

\begin{IEEEbiography}[{\biophoto{image/bio/zengdingchen.jpg}{60bp}{60bp}}]{Dingchen Zeng}
is currently pursuing a bachelor's degree in automation at the School of Automation Science and Electrical Engineering, Beihang University, Beijing, China. Current research interests include autonomous aerial robotics and embodied intelligence.
\end{IEEEbiography}


\begin{IEEEbiography}[{\biophoto{image/bio/quanquan.png}{13.75bp}{13.75bp}}]{Quan Quan}
(Senior Member, IEEE) received the B.S. and Ph.D. degrees in control science and engineering from Beihang University, Beijing, China, in 2004 and 2010, respectively. Since 2022, he has been a Professor with Beihang University, where he is currently with the School of Automation Science and Electrical Engineering. His research interests include reliable flight control, swarm intelligence, vision-based navigation, and health assessment.
\end{IEEEbiography}


